The Emperor's New Autofill Framework: A Security Analysis of Autofill on iOS and Android

Password managers help users more effectively manage their passwords, encouraging them to adopt stronger passwords across their many accounts. In contrast to desktop systems where password managers receive no system-level support, mobile operating systems provide autofill frameworks designed to integrate with password managers to provide secure and usable autofill for browsers and other apps installed on mobile devices. In this paper, we evaluate mobile autofill frameworks on iOS and Android, examining whether they achieve substantive benefits over the ad-hoc desktop environment or become a problematic single point of failure. Our results find that while the frameworks address several common issues, they also enforce insecure behavior and fail to provide password managers sufficient information to override the frameworks' insecure behavior, resulting in mobile managers being less secure than their desktop counterparts overall. We also demonstrate how these frameworks act as a confused deputy in manager-assisted credential phishing attacks. Our results demonstrate the need for significant improvements to mobile autofill frameworks. We conclude the paper with recommendations for the design and implementation of secure autofill frameworks.

==> storage.tex <==
\section{Password Storage}\label{sec:storage}

\begin{table*}[t]
	\begingroup
	\setuptable
	\renewcommand*{\prtline}{\hhline{~|-|-----|----|--|--|}}
	\renewcommand{\na}{-}
	
	\rowcolors{4}{gray!10}{}
	\begin{tabular}{l|l|lllrc|cccc|cc|cc|}
		\multicolumn{2}{l}{} \headline[2cm]
		& \hspace{1em}File type & Algorithm & MP KDF & \shortstack[l]{KDF\\Rounds} & \headrow{Requires strong MP} \headline[2cm]
		& \headrow{Username} & \headrow{URL} & \headrow{Creation time} & \headrow{Modification time} \headline[2cm] 
		& \headrow{User's email} & \headrow{User's settings} \headline[2cm] 
		& \headrow{Icons} & \headrow{Attachments}  \headline[2cm]
		\\ \hhline{~~|-----|----|--|--|}
		
		\multicolumn{1}{l}{} & System & \multicolumn{5}{c|}{Password encryption} & \multicolumn{8}{c|}{Metadata encryption} \\
		\hline
		
		%%%%%%%%%%%%%%%%%%%%%%%%%%%
		% App
		%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\hc&1Password		& SQLite w/ encrypted cells	& AES-256			& PBKDF2		& 100,000 	&\full
							&\full	&\full	&\none	&\none	&\full	&\full	&\full	&\na	\\
		\hc&Avast 			& SQLite w/ encrypted cells	& AES-256			& PBKDF2		& 10,240	&\none
							&\full	&\full	&\none	&\none	&\full	&\full	&\full	&\na	\\
		\hc&Bitwarden		& Encrypted SQLite file			& AES-256		& PBKDF2		& 100,001	&\full	
							&\full	&\full	&\full	&\full	&\full	&\full	&\full	&\na	\\
		\hc&Dashlane		& Encrypted SQLite file			& AES-256		& Argon2D		& 3		 	&\full	
							&\full	&\full	&\full	&\full	&\none	&\full	&\none	&\na	\\ \prtline
		\hc&Enpass			& SQLCipher						& AES-256		& PBKDF2		& 100,000	&\none	
							&\full	&\full	&\full	&\full	&\full	&\full	&\full	&\prt	\\
		\hc&iCloud Keychain	& SQLite w/ encrypted values	& AES-256		&\multicolumn{3}{c|}{Uses secure enclave}
							&\full	&\full	&\na	&\na	&\na	&\na	&\na	&\na	\\ 
		\hc&Keeper			& SQLite w/ encrypted cells		& AES-256		& PBKDF2		& 100,000	&\full
							&\full	&\full	&\none	&\none	&\none	&\full	&\full	&\full	\\
		\hc&Lastpass		& Custom encrypted file			& AES-256		& PBKDF2		&100,100	&\full
							&\full	&\full	&\full	&\full	&\full	&\full	&\na	&\na	\\ \prtline
		\hc&Lockwise 		& SQLCipher						& AES-256		&\multicolumn{3}{c|}{Uses secure enclave}
							&\full	&\full	&\full	&\full	&\full	&\full	&\na	&\na	\\
		\hc&Norton			& Custom encrypted file			& AES-256		& PBKDF2		& 1,000	 	&\full
							&\full	&\full	&\full	&\full	&\full	&\full	&\full	&\na	\\	
		\hc&RoboForm		& Custom encrypted file			& AES-256		& PBKDF2		& 4,000	 	&\none
							&\full	&\full	&\full	&\full	&\none	&\full	&\full	&\na	\\
		\hc&SafeInCloud	 	& Encrypted SQLite file			& AES-256		& PBKDF2		& 10,000	&\none
							&\full	&\full	&\full	&\full	&\full	&\full	&\full	&\na	\\
		\hc \headcol{-12}{AutoFill}
		\hc&StrongBox		& KeePass or PasswordSafe file	& AES-256		& Argon2D		& 2		 	&\none
							&\full	&\full	&\full	&\full	&\full	&\full	&\full	&\prt	\\ \hline

		%%%%%%%%%%%%%%%%%%%%%%%%%%%
		% Clipboard
		%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\hc&aWallet		 	& Custom encrypted file			& AES-256 		& SHA256		& 1,000	 	&\none
							&\full	&\full	&\full	&\full	&\full	&\full	&\na	&\full	\\
		\hc&My Passwords	& SQLite w/ encrypted cells	&AES-256		& PBKDF2		& 1,000		&\none
							&\full	&\full	&\full	&\full	&\full	&\full	&\na	&\na	\\
		\hc \headcol{-3}{Clipboard}
		\hc&PasswordSafe	& Encrypted SQLite file			& TwoFish-256	& PBKDF2		& 256		&\none
							&\full	&\full	&\full	&\full	&\full	&\full	&\na	&\na	\\	\hline

		%%%%%%%%%%%%%%%%%%%%%%%%%%%
		% Browser
		%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\hc&Chrome			& iCloud Keychain		&		&\multicolumn{3}{c|}{Uses secure enclave}
							&\none	&\none	&\none	&\none	&\none	&\na	&\na	&\na	\\
		\hc&Edge 			& iCloud Keychain		&		&\multicolumn{3}{c|}{Uses secure enclave}
							&\none	&\none	&\none	&\none	&\none	&\na	&\na	&\na	\\
		\hc \headcol{-3}{Browser}
		\hc&Firefox		 	& SQLCipher			 	&		&\multicolumn{3}{c|}{Uses secure enclave}
							&\full	&\full	&\full	&\full	&\full	&\full	&\na	&\na	\\	\hline
	\end{tabular}
	
	\begin{tabular}{llll}
		\full~~Secure behavior &
		\prt~~Partially secure behavior &
		\none~~Insecure behavior &
		\na~~Not stored
	\end{tabular}

	\begin{tabular}{ll}
		MP = Master Password &
		KDF = Key Derivation Function
	\end{tabular}

	\caption{Overview of Password Vault Encryption}
	\label{tab:storage}
	\endgroup
\end{table*}

While iOS does prevent apps from reading files (e.g., password vaults) for other apps, there is always the potential that an iOS bug could be leverage to allow a malicious app to read the password vault.
As such, it is important that passwords and metadata stored in the vault are properly secured.
To evaluate password storage security, we first searched the file system on our jailbroken device to find the password vault file used by each password manager.
We then used a combination of approaches (reverse engineering applications, inspecting system calls, looking at source code, communicating with the developer, and reviewing documentation) to determine the encryption algorithm used to protect this file, including the key derivation function (KDF) used to convert the user's master password into an encryption key that protects their vault.
Table~\ref{tab:storage} summarizes our findings.

\subsection{Password Encryption}
There were a variety of file types used to stored credentials: SQLite database with encrypted cells (1Password, Avast, iCloud Keychain, Keeper, MyPasswords), a SQLite database that was in an encrypted file (Bitwarden, Dashlane, SafeInCloud, PasswordSafe), SQLCipher (Lockwise, Firefox), and other custom encrypted files (Enpass, LastPass, Norton, RoboForm, aWallet).
Chrome and Edge both store their passwords in the iCloud Keychain, but also maintain a separate unencrypted database with additional metadata.

Other than PasswordSafe which encrypts its password vault using TwoFish-256, all password managers encrypt the password vault using AES-256.
Five of the password managers (iCloud Keychain, Lockwise, Chrome, Edge, Firefox) generate a random encryption key and store it using iOS's secure enclave.
While the details of the secure enclave are out of scope for this paper, we note that it provides adequate (if not ideal) protection for the encryption keys~\cite{green2014why}.
The other password managers derive an encryption key by feeding the user's master password to a key derivation function (KDF).

Two password managers (Dashlane, StrongBox) support Argon2D, a memory-hard KDF that is more resistant to offline attacks than PBKDF2.
aWallet uses SHA256 as its KDF, though with only 1,000 rounds, which is less than ideal.
The remaining password managers use PBKDF2, though several use 1,000 or fewer rounds(Norton, MyPasswords, PasswordSafe), which, similar to SHA256, is less than ideal.

%LastPass: 12 characters (1 number, 1 lowercase, 1 uppercase, not email)
%Norton: zxcvbn
%1password: 10 characters (no composition)
%Keeper: 10 characters (no composition)
%Dashlane: 8 characters (1 number, 1 uppercase, 1 lowercase)
%Bitwarden: 8 characters (no composition)
%Roboform: 4 characters (at least 4 non-numeric)
%Awallet: 4 characters (no composition)
%MyPasswords: 4 characters (no composition)
%Avast: 4 characters (no composition)
%SafeInCloud: 4 characters (no composition)
%StrongBox: At least 1 character
%PasswordSafe: At least 1 character
%Enpass: At least 1 character

For the password managers that rely on a master password, most do not require strong master passwords, making them vulnerable to offline attack and in some cases even online attacks for vaults that are synced online.
Only six (1Password, Bitwarden, Dashlane, Keeper, Lastpass) met the NIST guidelines for passwords~\cite{grassi2020digital}, though most just barely met these requirements which may not be sufficient for high-value secrets like a master password.
Five (Avast, RoboForm, SafeInCloud, aWallet, MyPasswords) allow four character passwords and three (Enpass, StrongBox, PasswordSafe) allow one character passwords.

\subsection{Metadata Privacy}
Other than Chrome and Edge, which do not protect any metadata, all password managers encrypted the username and url associated with a given password.
The protection of other metadata was less consistent.
Five (1Password, Avast, Keeper, Chrome, Edge) stored the creation and modification times in plaintext and
five (Dashlane, Keeper, RoboForm, Chrome, Edge) stored the email associated with the password manager in plaintext.
Enpass does store some user settings unencrypted (e.g., KDF rounds), though they are not private and any attempt to change these settings would either cause Enpass to fail to load or be automatically overwritten the next time Enpass was loaded.

Almost half of the password managers (1Password, Avast, Bitwarden, Dashlane, Enpass, Keeper, Norton, RoboForm) store icons for each of the stored credentials.
Dashlane fails to encrypt these icons which could allow an adversary to learn what websites a user visits~\cite{oesch2020that}.
Four password managers (Enpass, Keeper, StrongBox, aWallet) offer to store attachments for users, though Enpass and StrongBox leave an unencrypted version of the attachment in the \texttt{/tmp} folder.

\subsection{Comparison to Desktop Managers}\
Compared to desktop password managers~\cite{oesch2020that}, we find that browser-based password managers are more secure due to their use of iOS's secure enclave to store encryption keys for their password vaults.
We also find that managers generally use the same KDF settings on both desktop and iOS.
In regards to metadata privacy, we find that results are mixed for both desktop and iOS, with some password managers providing good protections and others providing poor protections.

